Towards Robust Multimodal Open-set Test-time Adaptation via Adaptive Entropy-aware Optimization

Test-time adaptation (TTA) has demonstrated significant potential in addressing distribution shifts between training and testing data. Open-set test-time adaptation (OSTTA) aims to adapt a source pre-trained model online to an unlabeled target domain that contains unknown classes. This task becomes more challenging when multiple modalities are involved. Existing methods have primarily focused on unimodal OSTTA, often filtering out low-confidence samples without addressing the complexities of multimodal data. In this work, we present Adaptive Entropy-aware Optimization (AEO), a novel framework specifically designed to tackle Multimodal Open-set Test-time Adaptation (MM-OSTTA) for the first time. Our analysis shows that the entropy difference between known and unknown samples in the target domain strongly correlates with MM-OSTTA performance. To leverage this, we propose two key components: Unknown-aware Adaptive Entropy Optimization (UAE) and Adaptive Modality Prediction Discrepancy Optimization (AMP). These components enhance the ability of model to distinguish unknown class samples during online adaptation by amplifying the entropy difference between known and unknown samples. To thoroughly evaluate our proposed methods in the MM-OSTTA setting, we establish a new benchmark derived from existing datasets. This benchmark includes two downstream tasks and incorporates five modalities. Extensive experiments across various domain shift situations demonstrate the efficacy and versatility of the AEO framework. Additionally, we highlight the strong performance of AEO in long-term and continual MM-OSTTA settings, both of which are challenging and highly relevant to real-world applications. Our source code is available at https://github.com/donghao51/AEO.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/abla_backbone.tex <==

\setlength{\tabcolsep}{2pt}

\begin{table}[t!]
\centering
\resizebox{0.3\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c cccc  }
\hline

 \multicolumn{1}{c|}{{} } &\multicolumn{4}{c}{\textit{Mean} (I3D+TSN) }  
 \\
   \multicolumn{1}{c|}{{}} &  Acc$\uparrow$ & FPR95$\downarrow$ &  AUROC$\uparrow$ &  \multicolumn{1}{c}{H-score$\uparrow$} \\
\hline

 \multicolumn{1}{c|}{Source} &54.29 &74.63     &  62.14  & \multicolumn{1}{c}{\cellcolor{gray!30}38.39 }  \\

 \multicolumn{1}{c|}{Tent } &59.80 & 85.52    &   59.18 & \multicolumn{1}{c}{\cellcolor{gray!30}27.58 }  \\

  \multicolumn{1}{c|}{SAR}& 60.08& 82.67    & 62.86   & \multicolumn{1}{c}{\cellcolor{gray!30}30.40 }  \\

 \multicolumn{1}{c|}{OSTTA}&59.04 &84.42     &   63.06 & \multicolumn{1}{c}{\cellcolor{gray!30}28.41 }  \\

 \multicolumn{1}{c|}{UniEnt}&57.60 & 69.47    & 70.03   & \multicolumn{1}{c}{\cellcolor{gray!30}42.75 }  \\

 \multicolumn{1}{c|}{READ } & 58.00& 73.48    &66.89    & \multicolumn{1}{c}{\cellcolor{gray!30}40.89 }  \\



\multicolumn{1}{c|}{AEO (Ours)} &59.54      &66.87    &  74.14  & \multicolumn{1}{c}{\cellcolor{gray!30}\textbf{47.62} }\\

\hline

%%%%%%%%

\end{tabular} 
}
\caption{Ablation on \textbf{different backbones} using video and flow modalities on HAC dataset.}
\label{tab:abla_back} 
\end{table}

==> tables/abla_mix.tex <==

\setlength{\tabcolsep}{2pt}

\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c cccc cccc cccc cccc }
\hline

 \multicolumn{1}{c|}{{} } & \multicolumn{4}{c|}{Defocus (v) + Wind (a)} & \multicolumn{4}{c|}{Frost (v) + Traffic (a) } &\multicolumn{4}{c|}{Brightness (v) + Thunder (a)} & \multicolumn{4}{c}{Pixelate (v) + Rain (a)}
 \\
   \multicolumn{1}{c|}{{}} & Acc$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & \multicolumn{1}{c|}{H-score$\uparrow$} &  Acc$\uparrow$ & FPR95$\downarrow$ &  AUROC$\uparrow$ & \multicolumn{1}{c|}{H-score$\uparrow$}  & Acc$\uparrow$ & FPR95$\downarrow$ &  AUROC$\uparrow$ & \multicolumn{1}{c|}{H-score$\uparrow$} & Acc$\uparrow$ & FPR95$\downarrow$ & \multicolumn{1}{c}{AUROC$\uparrow$} & \multicolumn{1}{c}{H-score$\uparrow$} \\
\hline


 \multicolumn{1}{c|}{Source}   & 60.74 & 76.34  & \multicolumn{1}{c}{65.05}  & \multicolumn{1}{c|}{\cellcolor{gray!30}} &33.24  &89.08 & \multicolumn{1}{c}{57.17}& \multicolumn{1}{c|}{\cellcolor{gray!30}}  &78.97 & 56.45 & \multicolumn{1}{c}{80.43} & \multicolumn{1}{c|}{\cellcolor{gray!30}} & 70.63  &67.08  & \multicolumn{1}{c}{74.14} & \multicolumn{1}{c}{\cellcolor{gray!30}}  \\
 

 \multicolumn{1}{c|}{UniEnt}  &  63.79& 65.29  & \multicolumn{1}{c}{77.56}  & \multicolumn{1}{c|}{\cellcolor{gray!30}} & 45.24 &87.00 & \multicolumn{1}{c}{66.31}& \multicolumn{1}{c|}{\cellcolor{gray!30}}  & 77.84& 42.37 & \multicolumn{1}{c}{88.81} & \multicolumn{1}{c|}{\cellcolor{gray!30}} & 74.63  &47.53  & \multicolumn{1}{c}{86.52} & \multicolumn{1}{c}{\cellcolor{gray!30}}  \\
 
 \multicolumn{1}{c|}{READ}   &63.74  &56.11   & \multicolumn{1}{c}{79.41}  & \multicolumn{1}{c|}{\cellcolor{gray!30}} & 51.00 & 73.29& \multicolumn{1}{c}{71.87}& \multicolumn{1}{c|}{\cellcolor{gray!30}}  &78.03 & 38.84 & \multicolumn{1}{c}{89.36} & \multicolumn{1}{c|}{\cellcolor{gray!30}} &75.32   & 44.79 & \multicolumn{1}{c}{86.61} & \multicolumn{1}{c}{\cellcolor{gray!30}}  \\

 

 
 \multicolumn{1}{c|}{AEO (Ours)}   &  63.39& 53.89  & \multicolumn{1}{c}{82.38}  & \multicolumn{1}{c|}{\cellcolor{gray!30}} &  50.92&70.13 & \multicolumn{1}{c}{75.41}& \multicolumn{1}{c|}{\cellcolor{gray!30}}  & 77.82&35.61  & \multicolumn{1}{c}{91.11} & \multicolumn{1}{c|}{\cellcolor{gray!30}} &  75.32 &42.89  & \multicolumn{1}{c}{88.19} & \multicolumn{1}{c}{\cellcolor{gray!30}}  \\
\hline


%%%%%%%%%%%%%%%%


 \multicolumn{1}{c|}{{} }& \multicolumn{4}{c|}{JPEG (v) + Crowd (a) }   & \multicolumn{4}{c|}{ Gaussian (v) + Gaussian (a) } &  \multicolumn{4}{c|}{\textit{Mean} }
 \\
   \multicolumn{1}{c|}{{}} & Acc$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & \multicolumn{1}{c|}{H-score$\uparrow$} &  Acc$\uparrow$ & FPR95$\downarrow$ &  AUROC$\uparrow$ & \multicolumn{1}{c|}{H-score$\uparrow$}  & Acc$\uparrow$ & FPR95$\downarrow$ &  AUROC$\uparrow$ & \multicolumn{1}{c|}{H-score$\uparrow$} \\
\hline


 \multicolumn{1}{c|}{Source}  & 61.11    &74.92  & \multicolumn{1}{c}{66.34} & \multicolumn{1}{c|}{\cellcolor{gray!30}} & 61.68&74.68  & \multicolumn{1}{c}{69.77}& \multicolumn{1}{c|}{\cellcolor{gray!30}}   & & & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\cellcolor{gray!30}}  \\
 


 \multicolumn{1}{c|}{UniEnt} &   68.42  & 64.11 & \multicolumn{1}{c}{77.81} & \multicolumn{1}{c|}{\cellcolor{gray!30}} & 71.29& 51.00 & \multicolumn{1}{c}{84.85}& \multicolumn{1}{c|}{\cellcolor{gray!30}}   & & & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\cellcolor{gray!30}}  \\
 
 \multicolumn{1}{c|}{READ}   & 70.92    &  53.82& \multicolumn{1}{c}{81.56} & \multicolumn{1}{c|}{\cellcolor{gray!30}} & 72.87& 48.26 & \multicolumn{1}{c}{85.07}& \multicolumn{1}{c|}{\cellcolor{gray!30}}   & & & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\cellcolor{gray!30}}  \\

 \multicolumn{1}{c|}{AEO (Ours)} & 70.53    &50.89  & \multicolumn{1}{c}{83.63} & \multicolumn{1}{c|}{\cellcolor{gray!30}} &72.36 & 45.67 & \multicolumn{1}{c}{87.49}& \multicolumn{1}{c|}{\cellcolor{gray!30}}   & & & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{\cellcolor{gray!30}}  \\ 
\hline


\end{tabular} 
}
\vspace{-0.4cm}
\caption{Multimodal Open-set TTA with video and audio modalities on Kinetics-100-C, with corrupted video and audio modalities  (severity level 5). The corruptions for open-set data (HAC dataset) are mixed.}
\vspace{-0.2cm}
\label{tab:k100-mix} 
\end{table}

==> tables/abla_more_methods.tex <==
\setlength{\tabcolsep}{2pt}

\begin{table}[t]
\centering
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c cccc cccc }
\hline


 \multicolumn{1}{c|}{{} } & \multicolumn{4}{c|}{ HAC} & \multicolumn{4}{c}{EPIC-Kitchens }
 \\
   &Acc$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & \multicolumn{1}{c|}{H-score$\uparrow$} &  Acc$\uparrow$ & FPR95$\downarrow$ &  AUROC$\uparrow$ & \multicolumn{1}{c}{H-score$\uparrow$} \\
\hline

2LTTA& 59.86 & 82.17 & 63.25 & \multicolumn{1}{c|}{\cellcolor{gray!30}32.39}  & 47.43& 89.53& \multicolumn{1}{c}{61.30}  & \multicolumn{1}{c}{\cellcolor{gray!30}21.27}\\

COME& 62.44 & 83.00 &63.04  & \multicolumn{1}{c|}{\cellcolor{gray!30}31.61}  & 46.64&89.34 & \multicolumn{1}{c}{59.76}  & \multicolumn{1}{c}{\cellcolor{gray!30}21.91}\\


AEO (Ours) & 59.53&66.75  & 72.50 & \multicolumn{1}{c|}{\cellcolor{gray!30}\textbf{48.31}}  & 50.93  & 48.65 & \multicolumn{1}{c}{85.58} & \multicolumn{1}{c}{\cellcolor{gray!30}{\textbf{56.18}}} \\

\hline


\end{tabular} 
}
\vspace{-0.2cm}
\caption{{Comparison with more recent methods.}}

\label{tab:abla_more} 
\end{table}

==> tables/abla_pre.tex <==

\setlength{\tabcolsep}{2pt}

\begin{table}[t!]
\centering
\resizebox{0.55\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c cccc cccc }
\hline

 \multicolumn{1}{c|}{{} } &\multicolumn{4}{c|}{\textit{Mean} (SAM) } & \multicolumn{4}{c}{\textit{Mean} (SimMMDG) } 
 \\
   \multicolumn{1}{c|}{{}} & Acc$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ &  \multicolumn{1}{c|}{H-score$\uparrow$} &  Acc$\uparrow$ & FPR95$\downarrow$ &  AUROC$\uparrow$ &  \multicolumn{1}{c}{H-score$\uparrow$} \\
\hline

 \multicolumn{1}{c|}{Source} & 60.25& 79.54 &55.50  & \multicolumn{1}{c|}{\cellcolor{gray!30}33.87 }  & 58.87    &78.93   & 51.23  & \multicolumn{1}{c}{\cellcolor{gray!30}33.77 }  \\

 \multicolumn{1}{c|}{Tent }  & 61.24& 84.06 &59.04  & \multicolumn{1}{c|}{\cellcolor{gray!30}29.77 }  & 60.27   & 80.79  & 60.44  & \multicolumn{1}{c}{\cellcolor{gray!30}34.47 }  \\

  \multicolumn{1}{c|}{SAR} &62.23 & 77.80 &64.06  & \multicolumn{1}{c|}{\cellcolor{gray!30}35.78 }  & 60.54    &78.72   & 63.02  & \multicolumn{1}{c}{\cellcolor{gray!30}36.20 }  \\

 \multicolumn{1}{c|}{OSTTA}   & 61.19&77.49  &63.72  & \multicolumn{1}{c|}{\cellcolor{gray!30}38.24 }  &   59.80  & 77.87  & 63.59  & \multicolumn{1}{c}{\cellcolor{gray!30}36.59 }  \\

 \multicolumn{1}{c|}{UniEnt}  &61.32 &76.42  & 63.97 & \multicolumn{1}{c|}{\cellcolor{gray!30}36.90 }  &  62.44   &70.22   & 65.53  & \multicolumn{1}{c}{\cellcolor{gray!30}44.82 }  \\

 \multicolumn{1}{c|}{READ } &60.48 &71.74  &67.26  & \multicolumn{1}{c|}{\cellcolor{gray!30}43.86 }  &   59.93  & 70.16  &67.62   & \multicolumn{1}{c}{\cellcolor{gray!30}45.71 }  \\



\multicolumn{1}{c|}{AEO (Ours)} & 60.63 &  67.06 & 72.13   & \multicolumn{1}{c|}{\cellcolor{gray!30}\textbf{48.20} }  &     60.93 & 66.26   &70.86    & \multicolumn{1}{c}{\cellcolor{gray!30}\textbf{49.16} }\\

\hline

%%%%%%%%

\end{tabular} 
}
\caption{Ablation on \textbf{different pre-trained models} using video and audio modalities on HAC dataset.}
\label{tab:abla_pre} 
\end{table}

==> tables/cont.tex <==

\setlength{\tabcolsep}{2pt}

\begin{table}[t!]
\centering
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c cccc cccc }
\hline


 \multicolumn{1}{c|}{{} }& \multicolumn{4}{c|}{ \textit{Mean} (HAC) } &  \multicolumn{4}{c|}{\textit{Mean} (Kinetics100-C) }
 \\
   \multicolumn{1}{c|}{{}}  & Acc$\uparrow$ & FPR95$\downarrow$ &  AUROC$\uparrow$ & \multicolumn{1}{c|}{H-score$\uparrow$}  & Acc$\uparrow$ & FPR95$\downarrow$ &  AUROC$\uparrow$ & \multicolumn{1}{c|}{H-score$\uparrow$} \\
\hline


 \multicolumn{1}{c|}{Source} & 56.36 &78.24     &  56.68  & \multicolumn{1}{c|}{\cellcolor{gray!30}34.61 }    &  52.96&76.70  & \multicolumn{1}{c}{64.84} & \multicolumn{1}{c}{\cellcolor{gray!30}37.66}  \\
 
 \multicolumn{1}{c|}{Tent} &55.48 & 88.43    &   54.79 & \multicolumn{1}{c|}{\cellcolor{gray!30}23.13}  &  52.08&94.97  & \multicolumn{1}{c}{42.70}  & \multicolumn{1}{c}{\cellcolor{gray!30}11.74}\\

 \multicolumn{1}{c|}{SAR}   & 58.81& 87.81    & 58.92  & \multicolumn{1}{c|}{\cellcolor{gray!30}23.89 }  & 54.79 &95.47  & \multicolumn{1}{c}{36.42} & \multicolumn{1}{c}{\cellcolor{gray!30}10.89}\\

 \multicolumn{1}{c|}{OSTTA} &55.55 &84.36    &   61.06& \multicolumn{1}{c|}{\cellcolor{gray!30}29.77 }  & 57.53&92.36 & \multicolumn{1}{c}{50.62} & \multicolumn{1}{c}{\cellcolor{gray!30}17.05} \\

 \multicolumn{1}{c|}{UniEnt} &58.56 & 80.68    & 62.52  & \multicolumn{1}{c|}{\cellcolor{gray!30}32.30 }  &59.62  &68.33  & \multicolumn{1}{c}{77.99} & \multicolumn{1}{c}{\cellcolor{gray!30}46.43} \\
 
 \multicolumn{1}{c|}{READ}   & 57.76& 73.49    &65.00    & \multicolumn{1}{c|}{\cellcolor{gray!30}41.85 } & 61.10 & 48.29& \multicolumn{1}{c}{84.49}& \multicolumn{1}{c}{\cellcolor{gray!30}62.32}    \\

 \multicolumn{1}{c|}{AEO (Ours)}&60.08   &60.38    &  78.89  & \multicolumn{1}{c|}{\cellcolor{gray!30}\textbf{53.84} } & 58.74 &  42.62& \multicolumn{1}{c}{87.22}  & \multicolumn{1}{c}{\cellcolor{gray!30}\textbf{64.19}} \\ 
\hline


\end{tabular} 
}
\caption{\textbf{Continual} Multimodal Open-set TTA on HAC and Kinetics100-C datasets.}
\label{tab:cont} 
\end{table}

==> tables/hac_va_cont.tex <==

\setlength{\tabcolsep}{2pt}

\begin{table}[t!]
\centering
\resizebox{0.3\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c cccc  }
\hline

 \multicolumn{1}{c|}{{} } &\multicolumn{4}{c}{\textit{Mean} }  
 \\
   \multicolumn{1}{c|}{{}} &  Acc$\uparrow$ & FPR95$\downarrow$ &  AUROC$\uparrow$ &  \multicolumn{1}{c}{H-score$\uparrow$} \\
\hline

 \multicolumn{1}{c|}{Source} &56.36 &78.24     &  56.68  & \multicolumn{1}{c}{\cellcolor{gray!30}34.61 }  \\

 \multicolumn{1}{c|}{Tent } &55.48 & 88.43    &   54.79 & \multicolumn{1}{c}{\cellcolor{gray!30}23.13}  \\

  \multicolumn{1}{c|}{SAR}& 58.81& 87.81    & 58.92  & \multicolumn{1}{c}{\cellcolor{gray!30}23.89 }  \\

 \multicolumn{1}{c|}{OSTTA}&55.55 &84.36    &   61.06& \multicolumn{1}{c}{\cellcolor{gray!30}29.77 }  \\

 \multicolumn{1}{c|}{UniEnt}&58.56 & 80.68    & 62.52  & \multicolumn{1}{c}{\cellcolor{gray!30}32.30 }  \\

 \multicolumn{1}{c|}{READ } & 57.76& 73.49    &65.00    & \multicolumn{1}{c}{\cellcolor{gray!30}41.85 }  \\



\multicolumn{1}{c|}{AEO (Ours)} &60.08   &60.38    &  78.89  & \multicolumn{1}{c}{\cellcolor{gray!30}\textbf{53.84} }\\

\hline

%%%%%%%%

\end{tabular} 
}
\caption{\textbf{Continual} Multimodal Open-set TTA with video and audio modalities on HAC dataset (EPIC-Kitchens as OOD dataset).}
\label{tab:hac-va-cont} 
\end{table}

==> tables/hac_va_long.tex <==

\setlength{\tabcolsep}{2pt}

\begin{table}[t!]
\centering
\resizebox{0.3\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c cccc  }
\hline

 \multicolumn{1}{c|}{{} } &\multicolumn{4}{c}{\textit{Mean} }  
 \\
   \multicolumn{1}{c|}{{}} &  Acc$\uparrow$ & FPR95$\downarrow$ &  AUROC$\uparrow$ &  \multicolumn{1}{c}{H-score$\uparrow$} \\
\hline

 \multicolumn{1}{c|}{Source} &56.36 &78.24     &  56.68  & \multicolumn{1}{c}{\cellcolor{gray!30}34.61 }  \\

 \multicolumn{1}{c|}{Tent } &56.11& 97.02    &  47.82& \multicolumn{1}{c}{\cellcolor{gray!30}7.68}  \\

  \multicolumn{1}{c|}{SAR}& 57.68& 97.40   &45.60 & \multicolumn{1}{c}{\cellcolor{gray!30}6.87 }  \\

 \multicolumn{1}{c|}{OSTTA}&58.36 &88.00    &   63.22& \multicolumn{1}{c}{\cellcolor{gray!30}23.37 }  \\

 \multicolumn{1}{c|}{UniEnt}&50.91 & 80.27   & 59.85 & \multicolumn{1}{c}{\cellcolor{gray!30}30.07 }  \\

 \multicolumn{1}{c|}{READ } & 53.83& 77.10    &61.17& \multicolumn{1}{c}{\cellcolor{gray!30}36.97 }  \\



\multicolumn{1}{c|}{AEO (Ours)} &56.81  &50.53    &  79.64  & \multicolumn{1}{c}{\cellcolor{gray!30}\textbf{55.98} }\\

\hline

%%%%%%%%

\end{tabular} 
}
\caption{\textbf{Long-term} Multimodal Open-set TTA on HAC dataset.}
\label{tab:hac-va-long} 
\end{table}
